CBA: Contextual Quality Adaptation for Adaptive Bitrate Video Streaming (Extended Version)

Recent advances in quality adaptation algorithms leave adaptive bitrate (ABR) streaming architectures at a crossroads: When determining the sustainable video quality one may either rely on the information gathered at the client vantage point or on server and network assistance. The fundamental problem here is to determine how valuable either information is for the adaptation decision. This problem becomes particularly hard in future Internet settings such as Named Data Networking (NDN) where the notion of a network connection does not exist. In this paper, we provide a fresh view on ABR quality adaptation for QoE maximization, which we formalize as a decision problem under uncertainty, and for which we contribute a sparse Bayesian contextual bandit algorithm denoted CBA. This allows taking high-dimensional streaming context information, including client-measured variables and network assistance, to find online the most valuable information for the quality adaptation. Since sparse Bayesian estimation is computationally expensive, we develop a fast new inference scheme to support online video adaptation. We perform an extensive evaluation of our adaptation algorithm in the particularly challenging setting of NDN, where we use an emulation testbed to demonstrate the efficacy of CBA compared to state-of-the-art algorithms.

==> sections/3_1_contextual_bandits.tex <==
\section{Contextual Bandits}\label{sec:multi_armed_bandits}
\tdBA{TODO
\begin{itemize}
	\item motivate this by the need for a new algorithm which can use prior knowledge and assumes sparsity, since D>>T
    \item evaluation
    \item cite related work
    \begin{itemize}
            \item \cite{li2010} talk about this in a bit more detail
            \item \cite{dudik2011}(related work cb)
         \item \cite{agarwal2014} (related work cb)
         \item \cite{urteaga18} (related work variational)
    \end{itemize}
    \item go through bandit section and make it read nicer
    \item highlight contributions
    \item restructure paper with notes
\end{itemize}}

We model the problem of videostream adaptation as a contextual bandit problem. The contextual bandit problem is an extension to the mutli-armed bandit problem \cite{robbins1952}. The contextual bandit problem \cite{bubeck2012} or bandits with side information is an extension to the classic multi-armed bandit problem and can be seen as a sequential game.

At time step $t$ a learner observes a $D$ dimensional context variable $\mathbf{x}_{t,a} \in \mathbb{R}^D$ for a set of actions/arms $a \in \{1,\dots,K\}$. Then she chooses an action $a_t \in \mathcal{A}$ and observes for this the reward $r_{t,a_t}$. We consider here the case of a finite set of actions $\mathcal{A}=\{1,\dots,K\}$, meaning that there is a countable finite set of $K$ different arms to choose at each time step. The decision making is performed over a usually unknown time horizon $T$, \ie $t \in \{1, \dots, T\}$. Here, we model the contextual bandit problem under the linerization assumption \cite{auer2002} $\E[r_{t,a}]=\mathbf{x}_{t,a}^\top \pmb{\beta}_a^\ast$, meaning that we assume a linear parameter  $\pmb{\beta}_a^\ast \in \mathbb{R}^D$ is controlling the mean reward for each arm $a \in \mathcal{A}$. For evaluation purposes we introduce the regret of an algorithm as a measure of performance
\begin{equation}
R_T=\sum_{t=1}^T r_{t,a_t^\ast}-\sum_{t=1}^T r_{t,a_t},
\label{eq:regret}
\end{equation}
with $a_t^\ast=\argmax_{a \in \mathcal{A}} \mathbf{x}_{t,a}^\top \pmb{\beta}_a^{\ast}$. The regret compares the cumulative reward of the algorithm against the cumulative reward with hindsight.  
In order to develop algorithms with a small regret in the linear setting, many different strategies have been proposed. Such algorithms include techniques based on forced sampling \cite{bastani2015}, thompson sampling \cite{agrawal2013} and the upper confidence bound (UCB) \cite{auer2002,li2010,chu2011,krause2011}.

Since, we assume in the video streaming context a sparse regression coefficient vector we want to impose a sparsity inducing prior for the regression coefficients of the arms. To cope with the bandit setting we adapt the Bayes-UCB algorithm with liner bandits of \cite{kaufmann2012} to the contextual bandit setting.

\subsection{The Contextual Bayes-UCB Algorithm}
The Contextual Bayes-UCB (CB-UCB) selects in each round the arm $a$ which maximizes the index
\begin{equation}
q_a(t)=Q(1-\frac{1}{\alpha t}, \zeta_a^{t-1}),
\label{eq:idx_general}
\end{equation}
where $\zeta_a^{t-1}$ is the posterior distribution of the mean reward
\begin{equation}
\zeta_a^{t-1}=p(\mathbf{x}_{t,a}^\top \pmb{\beta}_a \mid \{(\mathbf{x}_{t^\prime,a}, r_{t^\prime,a}, a_{t^\prime}) \mid a_{t^\prime }=a\}_{t^\prime=1,\dots, t-1})
\label{eq:posterior_mean_reward}
\end{equation}
and $Q(t, \rho)$ is the quantile function associated to the distribution $\rho$, \ie $\mathbb{P}_\rho(X \leq Q(t, \rho))=t$. The parameter $\alpha$ is a width parameter for the UCB. The posterior $\zeta_a^{t-1}$ for each arm is calculated based on the set of previously observed data points, where arm $a$ was played $\{(\mathbf{x}_{t^\prime,a}, r_{t^\prime,a}, a_{t^\prime}) \mid a_{t^\prime }=a\}_{t^\prime=1,\dots, t-1}$. 

We will see that under approximate inference of the regression coefficients a Gaussian distribution for the posterior distribution of the regression coefficients can be obtained.
In the case of Gaussian distributed posterior distributions of the regression coefficents
$$p(\pmb{\beta}_a\mid \{(\mathbf{x}_{t^\prime,a}, r_{t^\prime,a}, a_{t^\prime}) \mid a_{t^\prime }=a\}_{t^\prime=1,\dots, t-1})=\NormalDis(\pmb{\beta}_a \mid \pmb{\mu}_{\pmb{\beta}_a}, \pmb{\Sigma}_{\pmb{\beta}_a}),$$
the index reduces to 
\begin{equation}
q_a(t)=\mathbf{x}_{t,a}^\top \pmb{\mu}_{\pmb{\beta}_a}+ Q\left(1-\frac{1}{\alpha t}, \NormalDis(\rho \mid 0,1)\right)\sqrt{\mathbf{x}_{t,a}^\top \pmb{\Sigma}_{\pmb{\beta}_a}\mathbf{x}_{t,a}},
\label{eq:idx_gaussian}
\end{equation}
where the quantile function is computed as $Q\left(1-\frac{1}{\alpha t}, \NormalDis(\rho \mid 0,1)\right)=\sqrt{2}\mathrm{erf}^{-1}(1-\frac{2}{ \alpha  t})$, with the inverse error function $\mathrm{erf}^{-1}(\cdot)$. The algorithm for CB-UCB is depicted in Fig.~\ref{fig:algorithms} Alg.~1.


%%%%%%%%%%%%%%%%%%%%%%%%% -all algorithms- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \removelatexerror
%%%%%%%%%%%%%%%%%%%%%%%%% -algorithm- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\columnwidth}
\centering
\begin{algorithm}[H]
\TitleOfAlgo{{\sc main-routine} CB-UCB with Gaussian Posterior}
\input{algorithms/algorithm_main}
\end{algorithm}
\end{subfigure}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
~ 
%%%%%%%%%%%%%%%%%%%%%%%%% -algorithm- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\columnwidth}
\centering
\begin{algorithm}[H]
\TitleOfAlgo{{\sc sub-routine} SVI}
\input{algorithms/algorithm_svi}
\end{algorithm}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% -algorithm- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\columnwidth}
\centering
\begin{algorithm}[H]
\TitleOfAlgo{{\sc sub-routine} VB}
\input{algorithms/algorithm_vb}
\end{algorithm}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
~
%%%%%%%%%%%%%%%%%%%%%%%%% -algorithm- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{\columnwidth}
\centering
\begin{algorithm}[H]
\TitleOfAlgo{{\sc sub-routine} OS-SVI}
\input{algorithms/algorithm_ossvi}
\end{algorithm}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{The CB-UCB Algorithm with the three Bayesian inference schemes for the regression coefficients}
\label{fig:algorithms}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Generative model of the linear rewards}
For the inference of the posterior \eqref{eq:posterior_mean_reward} we use Bayesian regression to infer the posterior distribution of the regression coefficients\footnote{For readability we drop the subscript $a$ of the regression coefficients $\pmb{\beta}_a$} $\pmb{\beta}=[\beta_1,\dots, \beta_D]^\top$.
For the data we use the set set of previously observed data points (\eg $M$ previously observed contexts $\mathbf{X}=[\mathbf{x}_1,\dots,\mathbf{x}_{M}]^\top$ and rewards $\mathbf{r}=[r_1,\dots,r_{M}]^\top$ when playing arm $a$. 
 Given the linear regression model $\mathbf{r}=\mathbf{X}\pmb{\beta}+\pmb{\epsilon},$ with i.i.d. noise $\pmb{\epsilon} \sim \NormalDis(\pmb{\epsilon} \mid \mathbf{0}, \mathbf{I}_M/\sigma^{-2})$ the regression response $\mathbf{r}$ follows the likelihood
$$p(\mathbf{r} \mid \pmb{\beta}, \sigma^{-2})=\prod_{m=1}^M p(r_m \mid \pmb{\beta}, \sigma^{-2}) =\prod_{m=1}^M  \NormalDis(r_m \mid\mathbf{x}_m^\top \pmb{\beta}, 1/\sigma^{-2}).$$
For the video streaming example we use a sparsity inducing prior over the regression coefficients $\pmb{\beta}$. Sparsity has been a major topic in statistical modeling and many Bayesian approaches have been proposed. Priors that induce sparsity include 'spike-and slab' priors \cite{ishwaran2005} 
and continuous shrinkage prior. Continuous shrinkage priors have the benefit that they are often computationally faster than 'spike-and-slab' type priors \cite{armagan2011}. We use here the Three Parameter Beta Normal (TPBN) continuous shrinkage prior introduced by \cite{armagan2011}, which generalizes diverse shrinkage priors such as the horseshoe prior \cite{carvalho2009}, the Strawderman-Berger prior \cite{strawderman1971,berger1980}, the normal-exponential-gamma prior \cite{griffin2007} and the normal-gamma prior \cite{griffin2010}.  The TPBN shrinkage prior puts on each regression coefficient $\beta_j$, $j \in \{1, \dots, D\}$, the following hierarchical prior\footnote{We use the shape and rate parametrization of the Gamma distribution.}
\begin{equation}
\begin{split}
&\beta_j \sim \NormalDis(\beta_j\mid0,\tau_j/\sigma^{-2}), \; \tau_j \sim \GammaDis(\tau_j\mid a_0, \lambda_j),\\
&\lambda_j \sim \GammaDis(\lambda_j\mid b_0,\phi),
\label{eq:tpbn_prior}
\end{split}
\end{equation}
where $\sigma^{-2}$ is the noise precision for the regression problem and $\tau_j$ is a continuous shrinkage parameter that shrinks $\beta_j$, as $\tau_j$ gets small.
The parameter $\lambda_j$ controls $\tau_j$ via the global shrinkage parameter parameter $\phi$. For appropriate hyper-parameter choice of $a_0$ and $b_0$ different shrinkage prior are obtained. For example for $a_0=1/2$, $b_0=1/2$ the horseshoe prior is obtained.

For the estimation of the global shrinkage parameter $\phi$ an additional hierarchy is used as $\phi \sim \GammaDis(\phi \mid 1/2, \omega)$ and  $\omega \sim \GammaDis(\omega \mid 1/2, 1)$. For the noise precision a gamma prior  is used $\sigma^{-2} \sim \GammaDis(\sigma^{-2}\mid c_0/2,d_0/2)$, with hyper parameters $c_0$ and $d_0$. The graphical model of this generative model is depicted in Fig.~\ref{fig:pgm}.


%%%%%%%%%%%%%%%%%%%%%%%%% -figure- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%[ht]
  \begin{center}
      \input{figures/pgm} 
  \end{center}
  \caption{Probabilistic Graphical Model}
  \label{fig:pgm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Variational Bayesian Inference}
Since, exact inference of the posterior distribution $p(\pmb{\beta}, \sigma^{-2}, \pmb{\tau}, \pmb{\lambda}, \phi, \omega \mid \mathbf{r})$ is intractable \cite{bishop2006}, we leverage approximate inference in form of variational Bayes (VB) for posterior inference. We use 
a mean field variational approximation, with $q(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega)=q(\pmb{\beta})q(\sigma^{-2})q( \pmb{\tau})q(\pmb{\lambda})q(\phi)q(\omega)$ for the approximate distribution. The variational distributions are obtained by minimizing the Kulback-Leibler (KL) divergence between the variational distribution and the intractable posterior distribution
\begin{equation}
\begin{split}
\mathrm{KL}&(q(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega) \Vert p(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega \mid \mathbf{r}))\\
=&\mathrm{E}_q[\log(q(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega))]\\
&-\mathrm{E}_q[\log(p(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega , \mathbf{r}))]\\
&\quad+\log(p(\mathbf{r}))
\end{split}
\label{eq:kl_divergence}
\end{equation}
By Jensen's inequality a lower bound on the marginal likelihood (evidence) can be found. 
\begin{equation}
\begin{split}
\mathcal{L}(q) &=\mathrm{E}_q[\log(p(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega , \mathbf{r}))]\\
&\quad-\mathrm{E}_q[\log(q(\pmb{\beta}, \sigma^{-2}, \pmb{\tau},\pmb{\lambda}, \phi, \omega))]\\
&\leq \log(p(\mathbf{r}))
\end{split}
\label{eq:elbo_general}
\end{equation}
The evidence lower bound (ELBO) $\mathcal{L}(q)$ can be used for solving the optimization problem over the KL divergence \eqref{eq:kl_divergence}, since maximizing $\mathcal{L}(q)$ is equivalent to minimizing the KL divergence. Using calculus of variations \cite{bishop2006}, the solution of the optimization problem can be found. The optimal variational distributions are\footnote{$\GIGDis(x\mid p,a,b)$ denotes the generalized inverse Gaussian distribution.}
\begin{equation}
\begin{split}
&q(\pmb{\beta})=\NormalDis(\pmb{\beta} \mid \pmb{\mu}_{\pmb{\beta}}, \pmb{\Sigma}_{\pmb{\beta}}),\; 
q( \sigma^{-2})= \GammaDis(\sigma^{-2} \mid c^\ast, d^\ast),\; \\
&q(\pmb{\tau}) = \prod_{j=1}^{D} \GIGDis(\tau_j \mid p_{\tau_j}, a_{\tau_j}, b_{\tau_j}),\;\\
 &q(\pmb{\lambda})=\prod_{j=1}^{D} \GammaDis(\lambda_j \mid a_{\lambda_j},b_{\lambda_j}),\; 
 q(\phi)= \GammaDis(\phi \mid a_{\phi}, b_{\phi}),\; \\
 &q(\omega)= \GammaDis(\omega \mid a_{\omega},b_{\omega}),
\end{split}
\label{eq:variational_distr}
\end{equation}
with the parameters of the variational distributions
\begin{equation}
\begin{split}
&\pmb{\mu}_{\pmb{\beta}}=(\mathbf{X}^\top \mathbf{X}+ \mathbf{T}^{-1})^{-1} \mathbf{X}^\top \mathbf{r}\\ 
&\pmb{\Sigma}_{\pmb{\beta}}=\langle \sigma^{-2}\rangle^{-1}  (\mathbf{X}^\top \mathbf{X}+ \mathbf{T}^{-1})^{-1},\\
&\mathbf{T}^{-1}=\diag(\langle \tau_1^{-1}\rangle,\dots,\langle \tau_D^{-1}\rangle),\;
   c^{\ast}=\frac{M+D+c_0}{2},\;\\
    &d^{\ast}=(\mathbf{r}^\top \mathbf{r} - 2\mathbf{r}^\top\mathbf{X}\langle \pmb{\beta}\rangle + \sum_{i=1}^t \mathbf{x}_i^\top \langle \pmb{\beta}\pmb{\beta}^{\top}\rangle \mathbf{x}_i  \\
    &\qquad +\sum_{j=1}^D \langle \beta_j^2 \rangle \langle \tau_j^{-1} \rangle+d_0)/2,\;\\
    &p_{\tau_j}=a_0-1/2,\;
a_{\tau_j}=2 \langle \lambda_j \rangle,\;
b_{\tau_j}=\langle \beta_j^2 \rangle \langle \sigma^{-2} \rangle,\;\\
&a_{\lambda_j}=a_0+b_0,\;
b_{\lambda_j}= \langle \tau_j \rangle + \langle \phi \rangle,\;\\
&a_{\phi}=Db_0+1/2,\;
b_{\phi}= \langle \omega \rangle + \sum_{j=1}^D \langle \lambda_j \rangle,\;\\
&a_{\omega}=1,\;
b_{\omega}= \langle \phi \rangle +1
\end{split}
\label{eq:variational_param}
\end{equation}
and the moments
\begin{equation}
\begin{split}
&\langle \pmb{\beta}\rangle=\pmb{\mu}_{\pmb{\beta}},\;
\langle \pmb{\beta} \pmb{\beta}^\top\rangle= \pmb{\Sigma}_{\pmb{\beta}}+\pmb{\mu}_{\pmb{\beta}}\pmb{\mu}_{\pmb{\beta}}^\top,\;\\ 
&\langle \sigma^{-2} \rangle = c^\ast / d^\ast,\;   
\langle \lambda_j \rangle= a_{\lambda_j}/b_{\lambda_j},\; 
\langle \phi \rangle = a_{\phi}/ b_{\phi},\;\\
&\langle \omega \rangle = a_{\omega}/b_{\omega},\;
v_j=\sqrt{2 a_{\tau_j} b_{\tau_j}},\;\\
&\langle \tau_j \rangle = \left(\frac{b_{\tau_j}}{a_{\tau_j}}\right)^{1/2} \frac{\mathrm{K}_{p_{\tau_j}+1}(v_j)}{\mathrm{K}_{p_{\tau_j}}(v_j)},\;\\ 
&\langle \tau_j^{-1} \rangle =\left(\frac{a_{\tau_j}}{b_{\tau_j}}\right)^{1/2} \frac{\mathrm{K}_{1-p_{\tau_j}}(v_j)}{\mathrm{K}_{-p_{\tau_j}}(v_j)},
\end{split}
\label{eq:variational_moments}
\end{equation}
where $K_p(\cdot)$ is the modified Bessel function of second kind.
The probabilistic graphical model of the mean field approximation for the generative model is shown in Fig~\ref{fig:pgm_mean_field}.

%%%%%%%%%%%%%%%%%%%%%%%%% -figure- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%[ht]
  \begin{center}
      \input{figures/pgm_mean_field} 
  \end{center}
  \caption{Probabilistic Graphical Model Mean Field}
   \label{fig:pgm_mean_field}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A local optimum of the ELBO can be found by cycling through the coupled moments of the variational distributions. This corresponds to a coordinate ascent algorithm on the ELBO.  The corresponding algorithm is shown in Fig.~\ref{fig:algorithms} Alg.~3. 

\subsection{Stochastic Variational Inference}
A different approach than the coordinate ascent algorithm is to use stochastic variational inference (SVI) \cite{hoffman2013}. The ELBO is optimized by the use of stochastic approximation \cite{robbins1951}.

In stochastic variational inference for the optimization of the ELBO the natural gradient is calculated.
%The natural gradient of a function $f(\cdot)$ w.r.t. a variable $\pmb{\eta}$  can be described by
%$$\hat{\nabla}_\pmb{\eta} f(\pmb{\eta})= G(\pmb{\eta})^{-1} \nabla_{\pmb{\eta}} f(\pmb{\eta}),$$
%where $G(\pmb{\eta})$ is the Fisher information matrix of $q(\eta)$. 
The natural gradient is obtained with respect to the natural parameters $\pmb{\eta}$ of the exponential family distribution \cite{wasserman2013} of the mean field variational distributions.

Consider the mean field approximation $q(\pmb{\theta})=\prod_m q(\theta_m)$, where each factor $q(\theta_m)$ is in the exponential  family. Then the probability density can be described as
$$q(\theta_m)=h(\theta_m) \exp\{\pmb{\eta}^\top \mathbf{S}(\theta_m)-A(\pmb{\eta})\}.$$
Here, $h(\theta_m)$ denotes the base measure, $\pmb{\eta}$ the natural parameters $\mathbf{S}(\theta_m)$ the sufficient statistics of the natural parameters and $A(\pmb{\eta})$ is the log-normalizer.

The natural gradient of the ELBO w.r.t. the natural parameters of the factorized variational distributions computes to \cite{hoffman2013}
$$ \hat{\nabla}_{\pmb{\eta}} \mathcal{L}=\tilde{\pmb{\eta}}-\pmb{\eta},$$
where $\tilde{\pmb{\eta}}=\mathrm{E}_q[\pmb{\eta}^{\mathrm{post}}]$ and $\pmb{\eta}^{\mathrm{post}}$ is the natural parameter of the posterior distribution. By using a gradient update the variational approximation can be found
\begin{equation}
\pmb{\eta}_{n+1}=\pmb{\eta}_{n}+ \gamma_n  \hat{\nabla}_{\eta} \mathcal{L}
\label{eq:gradient_update}
\end{equation}
Random subsampling of the data enables a stochastic approximation algorithm. For this $\tilde{\pmb{\eta}}$ is replaced by an unbiased estimate $\hat{\pmb{\eta}}$, which yields a stochastic gradient ascent algorithm on the ELBO
\begin{equation}
\pmb{\eta}_{n+1}=(1-\gamma_n)\pmb{\eta}_{n}+\gamma_n \hat{\pmb{\eta}}
\label{eq:stoch_gradient_update}
\end{equation}
For the case of the regression problem we sample one data point $(\mathbf{x}_m,r_m)$ from the set of observed data points and replicate it $M$ times to calculate $\hat{\eta}$. The intermediate estimates of the natural parameters are then obtained by
\begin{equation}
\begin{split}
&\hat{\pmb{\eta}}_{\pmb{\beta}}=\left(\langle\sigma^{-2}\rangle M \mathbf{x}_m r_m, -\frac{1}{2} \langle \sigma^{-2}\rangle (M \mathbf{x}_m \mathbf{x}_m^\top+\mathbf{T}^{-1})\right),\;  \\
&\hat{\pmb{\eta}}_{\sigma^{-2}}=\left(\frac{M+D+c_0}{2}-1, -(M r_m^2 - 2M r_m \mathbf{x}_m^\top \langle \pmb{\beta}\rangle\right.\\
&\qquad\qquad + \left.M \mathbf{x}_m^\top \langle \pmb{\beta}\pmb{\beta}^{\top}\rangle \mathbf{x}_m  +\sum_{j=1}^D \langle \beta_j^2 \rangle \langle \tau_j^{-1} \rangle+d_0)/2\right),\;  \\
&\hat{\pmb{\eta}}_{\tau_j}=\left(a_0-\frac{3}{2}, -\langle \lambda_j \rangle, \langle \beta_j^2 \rangle \langle\sigma^{-2}\rangle/2\right),\;\\
&\hat{\pmb{\eta}}_{\lambda_j}=\left(a_0+b_0-1, -\langle\tau_j\rangle-\langle\phi\rangle\right),\;\\
& \hat{\pmb{\eta}}_{\phi}=\left(D b_0 -\frac{1}{2},-\langle\omega\rangle -\sum_{j=1}^D \langle\lambda_j\rangle\right),\;\\
&\hat{\pmb{\eta}}_{\omega}=\left(0,-\langle\phi\rangle-1\right).
\end{split}
\label{eq:intermediate_estimates}
\end{equation}
The transformation from the natural parametrization to the variational parametrization is calculated using
\begin{equation}
\begin{split}
&\left(\pmb{\mu}_{\pmb{\beta}}, \pmb{\Sigma}_{\pmb{\beta}}\right)=\left(-\frac{1}{2}{\pmb{\eta}_{\pmb{\beta}}}^{-1}_2{\pmb{\eta}_{\pmb{\beta}}}_1,-\frac{1}{2} {\pmb{\eta}_{\pmb{\beta}}}^{-1}_2\right),\; \\
&\left(c^\ast,d^\ast\right)=\left( {{{\eta}_{\sigma^{-2}}}_1}+1,- {{{\eta}_{\sigma^{-2}}}_2}\right),\;\\
&\left(p_{\tau_j}, a_{\tau_j}, b_{\tau_j}\right)=\left({{\eta}_{\tau_j}}_1+1,-2{{\eta}_{\tau_j}}_2, 2{{\eta}_{\tau_j}}_3\right),\;\\
&\left(a_{\lambda_j}, b_{\lambda_j}\right)=\left({\eta_{\lambda_j}}_1+1, -{\eta_{\lambda_j}}_2\right),\;\\
& \left(a_{\phi}, b_{\phi}\right)=\left({\eta_{\phi}}_1+1, -{\eta_{\phi}}_2\right),\;\\
&\left(a_{\omega}, b_{\omega}\right)=\left({\eta_{\omega}}_1+1, -{\eta_{\omega}}_2\right)
\end{split}
\label{eq:natural_transform}
\end{equation} 
and the moments can be then be calculated with \eqref{eq:variational_moments}. For an algorithmic description of the SVI see Fig.~\ref{fig:algorithms} Alg.~2. 

\subsection{One Step Stochastic Variational Inference}
Usually in stochastic variational inference the stochastic approximation is iterated until convergence of the ELBO is reached. Since, this is computationally expensive we propose a one step stochastic variational inference (OS-SVI) algorithm for the bandit setting. 
In each round the learner observes a context and a reward $(\mathbf{x}_{t,a_t}, r_{t,a_t})$ based on the played action $a_t$.  This data point is used to update the variational paramerters of the $a$-th arm by going one step in the direction of the natural gradient of the ELBO. For this she calculates the intermediate estimates \eqref{eq:intermediate_estimates} based on $t$ replicates of the observed data point $(\mathbf{x}_{t,a_t},r_{t,a_t})$. The stochastic gradient update is then performed with \eqref{eq:stoch_gradient_update}. Transforming the natural parameters back to their corresponding parameteric form \eqref{eq:natural_transform} the updated mean $\pmb{\mu}_{\pmb{\beta}_{a_t}}$ and covariance matrix $\pmb{\Sigma}_{\pmb{\beta}_{a_t}}$ can be found. The one step SVI subroutine is described in Fig.~\ref{fig:algorithms} Alg.~4. 



\subsection{Numerical Evaulation}
For the numerical evaluation of the CB-UCB with TPBN prior, we create data based on linearization assumption. We use a problem a time horizon of $T=1000$, $D=20$ dimensions and $K=20$ arms. We use two experimental setups with a dense regression vector and a sparse regression coefficient vector (only $5$ regression coefficients are unequal to zero). We compare the CB-UCB using Variational Bayes, SVI and One Step SVI with two base-line algorithms LinUCB \cite{li2010} and CGP-UCB \cite{krause2011}. For the CGP-UCB we use for every arm independent linear kernels. The result for the full and the sparse setting are shown in Fig.~\ref{fig:regret_full} and Fig.~\ref{fig:regret_sparse}, respectively. In Fig~\ref{fig:table} the computation times of the simulations are shown.

%%%%%%%%%%%%%%%%%%%%%%%%% -figure- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%[!ht]
\centering
\includegraphics[width=\columnwidth]{regret_full.pdf}
\caption{Simulation dense linear model}
\label{fig:regret_full}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% -figure- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%[!ht]
\centering
\includegraphics[width=\columnwidth]{regret_sparse.pdf}
\caption{Simulation sparse linear model}
\label{fig:regret_sparse}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% -table- %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\input{figures/table_computation_time}
\caption{Computation times of the algorithms (Intel\textsuperscript{\textregistered} Xeon\textsuperscript{\textregistered} E5-2680 v3 @2.5Ghz )}
\label{fig:table}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For the sparse setting, which is to be expected for high dimensional problems, such as in the videostreaming case, the CB-UCB with variational Bayesian inference yields the smallest regret, see Fig.~\ref{fig:regret_sparse}. We observe in Fig.~\ref{fig:regret_full} that in the dense setting the CGP-UCB obtains a high performance, closely followed by the  the CB-UCB with variational Bayesian inference. The CGP-UCB is performing well, since Gaussian process regression with linear kernel corresponds to a dense Bayesian regression with margenalized regression coefficients, which is the model under which the dense data has been created. 
Unfortunately, the computation times, see \ref{fig:table}, for both the variational Bayesian inference and  CGP-UCB baseline are quite high. This even magnifies as the dimensions of the context grows, since the computational bottle neck of the algorithms are mutliple matrix inversions of size $D \times D$. Since, the decision making has to be made in the order of \tdBA{Put videostream time reference here}, neither the CB-UCB with VB or CGP-UCB can be computed in the time restrictions. For this reason we resort to the OS-SVI inference algorithm, which beats the fast LinUCB baseline algorithm, but stays still in the same magnitude of computation time\footnote{For updating CB-UCB with OS-SVI  or LinUCB we only have to invert a $D \times D$ matrix once after a decision.}, rendering the video stream adaptation feasible.

